Consistent Recurrent Neural Networks for 3D Neuron Segmentation

We present a recurrent network for the 3D reconstruction of neurons that sequentially generates binary masks for every object in an image with spatio-temporal consistency. Our network models consistency in two parts: (i) local, which allows exploring non-occluding and temporally-adjacent object relationships with bi-directional recurrence. (ii) non-local, which allows exploring long-range object relationships in the temporal domain with skip connections. Our proposed network is end-to-end trainable from an input image to a sequence of object masks, and, compared to methods relying on object boundaries, its output does not require post-processing. We evaluate our method on three benchmarks for neuron segmentation and achieved state-of-the-art performance on the SNEMI3D challenge.

==> latex/05a_exp_em.tex <==
\input{latex/fig-tex/fig_exp_em.tex}
%\subsection{3D Instance Segmentation in Connectomics}
\subsection{Comparing with State-of-the-art Methods}
%\mysubsubsection{Datasets}

\bfsection{EM Dataset}
We use three benchmark datasets that have diverse properties (Table~\ref{tab:datasets}).
SNEMI3D~\cite{kasthuri2015saturated} is an SEM dataset that was imaged in mouse cortex and was used for the SNEMI challenge~\cite{snemi}. This dataset is anisotropic with the $x,y,z$ resolution ($6\times 6\times 30$ nm). Both the training and test data has $1024\times 1024\times 100$ voxels.

FIBSEM~\cite{fibsem} is isotropic, i.e., the $x, y, z$ resolutions for each voxel are all the same ($10$ nm). The training and test volumes in our experiments have the same size, $500\times 500\times 500$ voxels.

FIBER is an in-house dataset extracted from a mouse cerebellum.
Although the neurite segmentation is simple cylinders, there can be false merges on 2D sections.  We extracted a volume of size $1024\times1024\times105$ voxels.

\bfsection{Methods in Comparison}
We compare our full model with the state-of-the-art methods FFN~\cite{ffn} and waterz~\cite{funke}.
For FFN, we can only compare our method on the public SNEMI3D with their submission, as we are unable to produce satisfying results due to the high computational cost.
For waterz, we use the publicly available implementation from the author and use the suggested hyper-parameters from the original paper.

\bfsection{Evaluation Metrics}
For neuron segmentation, we analyze our experimental results with the Adaptive Rand Index (ARI)~\cite{randindex} to measure the similarity between two data clusters.  
The error is defined as one minus the maximal F-score of the Rand index.
Lower ARI score corresponds to better segmentation quality.

\bfsection{Quantitative Results}
(Table \ref{tab:benchmark}).
 On SNEMI3D, our method achieves a 0.035 ARI score surpassing the human accuracy, where methods with super-human accuracy are usually considered comparable with a minor difference. 
 For waterz, our method consistently outperforms it on all three datasets. For a fair comparison, we start from the same 2D segmentation as ours. Although both methods start from the same initial segmentation, our STRU-Net model can find better segments to link through learning and correct the error in initial segmentation through the forward-backward consistency check.

%\mysubsubsection{Quantitative Results}
\bfsection{Qualitative Results}
We show qualitative results and error cases for SNEMI3D, FIBSEM and FIBER datasets in Fig. ~\ref{fig:qualitative}. The first row shows the ground truth, the second row the waterz results, and the last row is our method results.  We show merge errors in Fig. ~\ref{fig:qualitative}(a), split errors in Fig. ~\ref{fig:qualitative}(b), and in Fig. ~\ref{fig:qualitative}(c),  we show the robustness of our system with propagation of labels across missing segments.
\input{latex/tab-tex/tab_em_result.tex}


\bfsection{Runtime Analysis}
One big advantage of the proposed method is fast. Our method has been designed to scale to large datasets in the TB range efficiently.   On a volume of ${100 \times 1024 \times 1024}$, the inference time of our STRU network is $120$ seconds per frame, for a total of $1200$ seconds.  These times reflect the total time to extract all the neuron structures simultaneously.  In comparison to FFN, this is 3$\times$ speedup during inference.  The FFN model trained by us takes 61 minutes on the same test volume of the SNEMI dataset.

==> latex/05c_ablation.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{lcc}
\hline
% \multicolumn{5}{|c|}{Cell spanning three columns} \\
 Model & Accuracy & Inference Time (seconds)  ~~ \\
\hline%\hline
%PNI~\cite{superhuman}  & N/A &  0.024 & N/A\\ %\hline
ST      & 0.15 & 520.0 \\
STC (S) & 0.08 & 640.0 \\
STC (L) & 0.03 & 605.0 \\
STC (SL) & 0.02 & 660.0 \\
  \hline
\end{tabular}
\end{center}
\caption{Ablation study evaluated on our training and validation set of Fiber dataset.  We show accuracy showing the Rand Error results, and inference time for each model. }
\label{tab:ablation_studies}
\end{table}
% \input{latex/fig-tex/fig_app.tex}
\bfsection{Spatial vs Temporal Recurrence}
We first test the use of spatial and temporal recurrence.  In Table \ref{tab:ablation_studies}, Rows 1, 2, and 3 shows the results of spatial, temporal, and spatial-temporal recurrence.  In the table we can see that combining spatial and temporal recurrency yields lower Rand Error for the model STRU-ST.

==> latex/fig-tex/fig_architecture.tex <==
% \begin{figure}[htb]
% \begin{minipage}[b]{1.0\linewidth}
%   \centering \centerline{\includegraphics[clip, trim=5.0cm 0.0cm 5.0cm 0.0cm, width=\textwidth]{latex/fig/architecture.pdf}}
% \end{minipage}
% \vspace{-0.5in}
% \caption{\label{fig:architecture}

% }
% \end{figure}


\begin{figure}[htb]
\centering 
\begin{minipage}[b]{0.9\linewidth}
   \centerline{\includegraphics[clip, trim=5.5cm 2.0cm 6.5cm 2.0cm, width=\textwidth]{latex/fig/architecture_jpg}}
\end{minipage}
\caption{
 Our proposed architecture for multi-neuron segmentation showing a single forward pass predicting the first object $S_{t,o}$ of the first frame $I_t$ of a sequence. 
}
\label{fig:architecture}
\end{figure}

% $L_{t,o}$ 
% Resnet50
% Label map
% STC Conv LSTM
% N = 128

% N/2
% N/4
% N/8
% Decoder
% 2048
% 1024
% 512
% 256
% 64
% 32

% \begin{figure}[htb]
% \centering 
% \begin{minipage}[b]{0.9\linewidth}
%   \centerline{\includegraphics[clip, trim=15.0cm 6.5cm 15.0cm 6.5cm, width=\textwidth]{latex/fig/architecture.pdf}}
% \end{minipage}
% \caption{
% % Our proposed architecture for instance segmentation of multiple neurons.  (a) A sequence is encoded by a Resnet50 at multiple resolution.  (b) A decoder processes input feature maps and a multi-resolution label map with bi-directional recurrence to extract neurons across a sequence.

% % Using a conditional encoder-decoder architecture, a multi-dimensional feature map carrying object distribution information from a reference label map ($Labels_{i+1}$) is used to condition object decoding.  The encoder learns features of an input image sequence at multiple resolutions. And the decoder integrates the features and the object distribution features to propagate objects across the sequence.
% khkljh
% }
% \label{fig:architecture}
% \end{figure}


==> latex/fig-tex/fig_exp_em.tex <==
\begin{figure*}[t]
\centering 
\begin{minipage}[b]{0.9\linewidth}
   \centerline{\includegraphics[clip, trim=0.5cm 0.5cm 0.5cm 0.5cm, width=\textwidth]{latex/fig/combined_qualitative_results.pdf}}
\end{minipage}
\caption{
Qualitative results on SNEMI, FIBSEM, and FIBER datasets. Compared to waterz~\cite{funke}, our method is robust against (a) merge errors, (b) split errors. (c) Even when segments are missing, our method can propagate labels as long as there's evidence of consistent structure.      
}
\label{fig:qualitative}
\end{figure*}

